LiveView: Dynamic Target-Centered MPI for View Synthesis

Existing Multi-Plane Image (MPI) based view-synthesis methods generate an MPI aligned with the input view using a fixed number of planes in one forward pass. These methods produce fast, high-quality rendering of novel views, but rely on slow and computationally expensive MPI generation methods unsuitable for real-time applications. In addition, most MPI techniques use fixed depth/disparity planes which cannot be modified once the training is complete, hence offering very little flexibility at run-time. We propose LiveView - a novel MPI generation and rendering technique that produces high-quality view synthesis in real-time. Our method can also offer the flexibility to select scene-dependent MPI planes (number of planes and spacing between them) at run-time. LiveView first warps input images to target view (target-centered) and then learns to generate a target view centered MPI, one depth plane at a time (dynamically). The method generates high-quality renderings, while also enabling fast MPI generation and novel view synthesis. As a result, LiveView enables real-time view synthesis applications where an MPI needs to be updated frequently based on a video stream of input views. We demonstrate that LiveView improves the quality of view synthesis while being 70 times faster at run-time compared to state-of-the-art MPI-based methods.

==> sections/figures/camera_layout.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth, height=0.38\textwidth]{images/camera_config.pdf}\par
    \caption{We have three different camera configuration for training and testing.
    Different camera configurations were used to compare against different algorithms as mentioned in the paper.}
    \label{fig:camera_config}
\end{figure}

==> sections/figures/supplementary_10_view.tex <==
\begin{figure*}
     \centering
     \begin{subfigure}
         \centering
         \includegraphics[width=\textwidth]{images/comparison_10_view_scene_1.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}
         \centering
         \includegraphics[width=\textwidth]{images/comparison_10_view_scene_2.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}
         \centering
         \includegraphics[width=\textwidth]{images/comparison_10_view_scene_5.pdf}
     \end{subfigure}
     \begin{subfigure}
         \centering
         \includegraphics[width=\textwidth]{images/comparison_10_view_scene_6.pdf}
     \end{subfigure}
     \caption{Comparison of 10 input configuration using our dynamic target-centered view synthesis and static input-centered LLFF~\cite{mildenhall2019local}. Inset shows a zoom in with the absolute difference map below it.}
    \label{fig:10_view}
\end{figure*}

% \begin{figure*}
%      \centering
%      \begin{subfigure}
%          \centering
%          \includegraphics[width=\textwidth]{images/comparison_10_view_scene_0.pdf}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}
%          \centering
%          \includegraphics[width=\textwidth]{images/comparison_10_view_scene_1.pdf}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}
%          \centering
%          \includegraphics[width=\textwidth]{images/comparison_10_view_scene_2.pdf}
%      \end{subfigure}
%      \begin{subfigure}
%          \centering
%          \includegraphics[width=\textwidth]{images/comparison_10_view_scene_3.pdf}
%      \end{subfigure}
%      \label{fig:10_view_0_3}
% \end{figure*}

% \begin{figure*}
%      \centering
%      \begin{subfigure}
%          \centering
%          \includegraphics[width=\textwidth]{images/comparison_10_view_scene_4.pdf}
%      \end{subfigure}
%      \begin{subfigure}
%          \centering
%          \includegraphics[width=\textwidth]{images/comparison_10_view_scene_5.pdf}
%      \end{subfigure}
%      \begin{subfigure}
%          \centering
%          \includegraphics[width=\textwidth]{images/comparison_10_view_scene_6.pdf}
%      \end{subfigure}
%      \begin{subfigure}
%          \centering
%          \includegraphics[width=\textwidth]{images/comparison_10_view_scene_7.pdf}
%      \end{subfigure}
%         \label{fig:10_view_4_7}
% \end{figure*}

% \begin{figure*}[ht!]
%      \centering
%      \begin{subfigure}
%          \centering
%          \includegraphics[width=\textwidth]{images/comparison_10_view_scene_8.pdf}
%      \end{subfigure}
%     \caption{Comparison of 10 input configuration using our dynamic target-centered view synthesis and static input-centered LLFF~\cite{mildenhall2019local}. Inset shows a zoom in with the absolute difference map below it.}
%     \label{fig:10_view_8_8}
% \end{figure*}

==> sections/figures/supplementary_5_view.tex <==
\begin{figure*}
     \centering
     \begin{subfigure}
         \centering
         \includegraphics[width=\textwidth]{images/comparison_5_view_scene_2.pdf}
     \end{subfigure}
     \begin{subfigure}
         \centering
         \includegraphics[width=\textwidth]{images/comparison_5_view_scene_3.pdf}
     \end{subfigure}
     \begin{subfigure}
         \centering
         \includegraphics[width=\textwidth]{images/comparison_5_view_scene_4.pdf}
     \end{subfigure}
     \begin{subfigure}
         \centering
         \includegraphics[width=\textwidth]{images/comparison_5_view_scene_5.pdf}
     \end{subfigure}
        \caption{Comparison of our dynamic target-centered view synthesis and static input-centered view synthesis using both, Stereo Magnification ~\cite{zhou2018stereo} Local LF (base network for LLFF~\cite{mildenhall2019local}). Results are shown for 5 view input configuration. Inset shows a zoom in with the absolute difference map below it.}
        \label{fig:5_view}
\end{figure*}



% \begin{figure*}
%      \centering
%      \begin{subfigure}
%          \centering
%          \includegraphics[width=\textwidth]{images/comparison_5_view_scene_0.pdf}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}
%          \centering
%          \includegraphics[width=\textwidth]{images/comparison_5_view_scene_1.pdf}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}
%          \centering
%          \includegraphics[width=\textwidth]{images/comparison_5_view_scene_2.pdf}
%      \end{subfigure}
%      \begin{subfigure}
%          \centering
%          \includegraphics[width=\textwidth]{images/comparison_5_view_scene_3.pdf}
%      \end{subfigure}
%      \begin{subfigure}
%          \centering
%          \includegraphics[width=\textwidth]{images/comparison_5_view_scene_4.pdf}
%      \end{subfigure}
%      \label{fig:5_view_0_4}
% \end{figure*}

% \begin{figure*}
%      \centering
%      \begin{subfigure}
%          \centering
%          \includegraphics[width=\textwidth]{images/comparison_5_view_scene_5.pdf}
%      \end{subfigure}
%      \begin{subfigure}
%          \centering
%          \includegraphics[width=\textwidth]{images/comparison_5_view_scene_6.pdf}
%      \end{subfigure}
%      \begin{subfigure}
%          \centering
%          \includegraphics[width=\textwidth]{images/comparison_5_view_scene_7.pdf}
%      \end{subfigure}
%      \begin{subfigure}
%          \centering
%          \includegraphics[width=\textwidth]{images/comparison_5_view_scene_8.pdf}
%      \end{subfigure}
%         \caption{Comparison of our dynamic target-centered view synthesis and static input-centered view synthesis using both, Stereo Magnification ~\cite{zhou2018stereo} Local LF (base network for LLFF~\cite{mildenhall2019local}). Results are shown for 5 view input configuration. Inset shows a zoom in with the absolute difference map below it.}
%         \label{fig:5_view_5_8}
% \end{figure*}
